What Makes a Code Review Useful to OpenDev Developers? An Empirical Investigation

Context: Due to the association of significant efforts, even a minor improvement in the effectiveness of Code Reviews(CR) can incur significant savings for a software development organization. Aim: This study aims to develop a finer grain understanding of what makes a code review comment useful to OSS developers, to what extent a code review comment is considered useful to them, and how various contextual and participant-related factors influence its usefulness level. Method: On this goal, we have conducted a three-stage mixed-method study. We randomly selected 2,500 CR comments from the OpenDev Nova project and manually categorized the comments. We designed a survey of OpenDev developers to better understand their perspectives on useful CRs. Combining our survey-obtained scores with our manually labeled dataset, we trained two regression models - one to identify factors that influence the usefulness of CR comments and the other to identify factors that improve the odds of `Functional' defect identification over the others. Key findings: The results of our study suggest that a CR comment's usefulness is dictated not only by its technical contributions such as defect findings or quality improvement tips but also by its linguistic characteristics such as comprehensibility and politeness. While a reviewer's coding experience positively associates with CR usefulness, the number of mutual reviews, comment volume in a file, the total number of lines added /modified, and CR interval has the opposite associations. While authorship and reviewership experiences for the files under review have been the most popular attributes for reviewer recommendation systems, we do not find any significant association of those attributes with CR usefulness.

==> Sections/codes.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{tabular}{|p{3cm}|p{4cm}|p{4.5cm}|}
\hline
\textbf{Question}                                                                & \textbf{Code}                              & \textbf{Assigned category}                              \\ \hline
\multirow{23}{=}{Q8. In your opinion, what makes a code review useful?}    & Defect finding                    & \multirow{4}{*}{Find defects}                  \\ \cline{2-2}
                                                                        & Security issues                   &                                                \\ \cline{2-2}
                                                                        & Fulfill requirements              &                                                \\ \cline{2-2}
                                                                        & NIT/typos                         &                                                \\ \cline{2-3} 
                                                                        & Alternative implementation        & \multirow{3}{*}{Improve code quality}          \\ \cline{2-2}
                                                                        & Code optimization                 &                                                \\ \cline{2-2}
                                                                        & Improve documentation             &                                                \\ \cline{2-3} 
                                                                        & Respectful                        & \multirow{5}{=}{Timely and appropriate feedback}      \\ \cline{2-2}
                                                                        & Understandable                    &                                                \\ \cline{2-2}
                                                                        & Concrete example                  &                                                \\ \cline{2-2}
                                          & Constructive criticism            &                                                \\ \cline{2-2}
                                                & Timely feedback                   &                                                \\ \cline{2-3} 
                                                                        & Maintain design                   & \multirow{3}{*}{Maintainability}               \\ \cline{2-2}
                                                                        & Reduce maintenance cost           &                                                \\ \cline{2-2}
                                                                        & Readability                       &                                                \\ \cline{2-3} 
                                                                        & Knowledge transfer                & \multirow{3}{*}{Facilitates knowledge sharing} \\ \cline{2-2}
                                                                        & Mentoring                         &                                                \\ \cline{2-2}
                                                                        & Project awareness                 &                                                \\ \cline{2-3} 
                                                                        & Design suggestion                 & \multirow{3}{*}{Facilitates better design}     \\ \cline{2-2}
                                                                        & Wider context                     &                                                \\ \cline{2-2}
                                                                        & Question that leads better design &                                                \\ \cline{2-3} 
                                                                        & Positive encouragement            & Appreciate good work                           \\ \cline{2-3} 
                                                                        & Community building                & Helps community building                       \\ \hline
\end{tabular}


==> Sections/data_analysis_result.tex <==
\section{Results}




==> Sections/demographics.tex <==
%\section{Dataset and Demographics}
%\label{sec:demographics}
%To better understand the research context, following subsections provide an overview of our manually labeled dataset 

%\subsection{Dataset characteristics}

%\subsection{Respondents' Primary Project}
%\begin{table*}
	%\centering
    %\caption{Respondents' primary project}
    %\vspace{-8pt}
	%\label{table:primary_project}
	%\input{tables/primary_project}
    %\vspace{-8pt}
%\end{table*}
%In Table \ref{table:primary_project}, we present the question we asked the developers and the response of the developers. In total, 149 developers answered this question. Among them, 30 developers said that they have no primary open source project. They can be one time contributor or probably not committed to any open source project. 12 of the 149 developers said they have primary open source project, but they did not mention any name of their project. The rest 107 developers mentioned one or multiple open source project's name. As we conducted the survey on OpenStack developers, no surprising, 69 developers mentioned OpenStack as their primary project. 





==> tables/glm_mlr_combined.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\resizebox{.95\linewidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{l|rrr|rr|rr|rr|rr}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Factors}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Parameter estimates \\ for GLM\end{tabular}}                                 & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Likelihood ratio \\ test for MLR\end{tabular}}       & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Distinguish between\\ False Positive and\\ Functional class\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Distinguish between\\ Evolvability and\\ Functional class\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Distinguish between\\ Comprehension and\\ Functional class\end{tabular}} \\ \cline{2-12} 
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{\textbf{$\beta$}} & \multicolumn{1}{c|}{\textbf{$\chi^2$}} & \multicolumn{1}{c|}{\textit{\textbf{p-value}}} & \multicolumn{1}{c|}{\textbf{$\chi^2$}} & \multicolumn{1}{c|}{\textit{\textbf{p-value}}} & \multicolumn{1}{c|}{\textbf{$\beta$}}                     & \multicolumn{1}{c|}{\textit{\textbf{p-value}}}                     & \multicolumn{1}{c|}{\textbf{$\beta$}}                    & \multicolumn{1}{c|}{\textit{\textbf{p-value}}}                    & \multicolumn{1}{c|}{\textbf{$\beta$}}                   & \multicolumn{1}{c}{\textit{\textbf{p-value}}}                   \\ \hline
WRC                                           & \multicolumn{1}{r|}{.435}       & \multicolumn{1}{r|}{.352}                & .553                                           & \multicolumn{1}{r|}{4.706}                         & 0.195                                          & \multicolumn{1}{r|}{.555}                           & .647                                                               & \multicolumn{1}{r|}{-1.430}                        & .187                                                              & \multicolumn{1}{r|}{-1.633}                       & .196                                                            \\ \hline
PN                                            & \multicolumn{1}{r|}{-.002}      & \multicolumn{1}{r|}{.090}                & .764                                           & \multicolumn{1}{r|}{3.31}                          & 0.346                                          & \multicolumn{1}{r|}{.014}                           & .163                                                               & \multicolumn{1}{r|}{.005}                          & .425                                                              & \multicolumn{1}{r|}{-.002}                        & .777                                                            \\ \hline
CV                                            & \multicolumn{1}{r|}{-.198}      & \multicolumn{1}{r|}{2.403}               & .121                                           & \multicolumn{1}{r|}{110.36}                        & \textbf{0.000}                                 & \multicolumn{1}{r|}{1.374}                          & \textbf{.000}                                                      & \multicolumn{1}{r|}{1.847}                         & \textbf{0.000}                                                    & \multicolumn{1}{r|}{.706}                         & \textbf{.004}                                                   \\ \hline
CCR                                           & \multicolumn{1}{r|}{.042}       & \multicolumn{1}{r|}{.308}                & .579                                           & \multicolumn{1}{r|}{7.49}                          & 0.058                                          & \multicolumn{1}{r|}{.000}                           & .782                                                               & \multicolumn{1}{r|}{.000}                          & .051                                                              & \multicolumn{1}{r|}{.000}                         & .873                                                            \\ \hline
CL                                            & \multicolumn{1}{r|}{.0}  & \multicolumn{1}{r|}{1.175}               & .278                                           & \multicolumn{1}{r|}{0.73}                          & 0.866                                          & \multicolumn{1}{r|}{.000}                           & .922                                                               & \multicolumn{1}{r|}{.000}                          & .814                                                              & \multicolumn{1}{r|}{.000}                         & .416                                                            \\ \hline
CCY                                           & \multicolumn{1}{r|}{.000}       & \multicolumn{1}{r|}{.477}                & .490                                           & \multicolumn{1}{r|}{5.00}                          & 0.172                                          & \multicolumn{1}{r|}{-.001}                          & .082                                                               & \multicolumn{1}{r|}{-.001}                         & .059                                                              & \multicolumn{1}{r|}{-.001}                        & .129                                                            \\ \hline
RCS                                           & \multicolumn{1}{r|}{.005}       & \multicolumn{1}{r|}{.139}                & .709                                           & \multicolumn{1}{r|}{1.81}                          & 0.613                                          & \multicolumn{1}{r|}{-.014}                          & .418                                                               & \multicolumn{1}{r|}{-.040}                         & .531                                                              & \multicolumn{1}{r|}{-.044}                        & .734                                                            \\ \hline
MR                                            & \multicolumn{1}{r|}{-.120}      & \multicolumn{1}{r|}{5.273}               & \textbf{.022}                                  & \multicolumn{1}{r|}{11.40}                         & \textbf{0.010}                                 & \multicolumn{1}{r|}{-.001}                          & .197                                                               & \multicolumn{1}{r|}{-.001}                         & \textbf{.007}                                                     & \multicolumn{1}{r|}{.000}                         & .953                                                            \\ \hline
RCE                                           & \multicolumn{1}{r|}{.743}       & \multicolumn{1}{r|}{16.189}              & \textbf{.000}                                  & \multicolumn{1}{r|}{51.28}                         & \textbf{0.000}                                 & \multicolumn{1}{r|}{.000}                           & \textbf{.000}                                                      & \multicolumn{1}{r|}{.000}                          & .368                                                              & \multicolumn{1}{r|}{.000}                         & \textbf{.000}                                                   \\ \hline
PFRC                                          & \multicolumn{1}{r|}{-.553}      & \multicolumn{1}{r|}{9.418}               & \textbf{.002}                                  & \multicolumn{1}{r|}{10.41}                         & \textbf{0.015}                                 & \multicolumn{1}{r|}{.003}                           & \textbf{.006}                                                      & \multicolumn{1}{r|}{.002}                          & \textbf{.008}                                                     & \multicolumn{1}{r|}{.001}                         & .145                                                            \\ \hline
RI                                            & \multicolumn{1}{r|}{-.131}      & \multicolumn{1}{r|}{8.993}               & \textbf{.003}                                  & \multicolumn{1}{r|}{11.086}                        & \textbf{0.011}                                 & \multicolumn{1}{r|}{.000}                           & \textbf{.031}                                                      & \multicolumn{1}{r|}{.000}                          & .380                                                              & \multicolumn{1}{r|}{.000}                         & .251                                                            \\ \hline
IBF                                           & \multicolumn{1}{r|}{.034}       & \multicolumn{1}{r|}{.130}                & .718                                           & \multicolumn{1}{r|}{6.44}                          & 0.092                                          & \multicolumn{1}{r|}{-.893}                          & \textbf{.037}                                                      & \multicolumn{1}{r|}{.898}                          & \textbf{.002}                                                     & \multicolumn{1}{r|}{.517}                         & .126                                                            \\ \hline
INF                                           & \multicolumn{1}{r|}{-.072}      & \multicolumn{1}{r|}{.174}                & .676                                           & \multicolumn{1}{r|}{4.47}                          & 0.215                                          & \multicolumn{1}{r|}{.138}                           & .700                                                               & \multicolumn{1}{r|}{-.308}                         & .208                                                              & \multicolumn{1}{r|}{-.046}                        & .870                                                            \\ \hline
\end{tabular}
}

==> tables/likelihood_test.tex <==
\begin{tabular}{l|r|r|r}
\hline
\multicolumn{1}{c|}{\textbf{Variable}} & \multicolumn{1}{c|}{\textbf{AIC value}} & \multicolumn{1}{c|}{\textbf{Chi-Square}} & \multicolumn{1}{c}{\textbf{p-value}} \\ \hline
WRC                     & 4945.22                          & 4.706                                    & 0.195                                 \\ \hline
PN                             & 4943.83                         & 3.31                                   & 0.346                                 \\ \hline
CV                             & 5050.88                          & 110.36                                   & \textbf{0.000}                                 \\ \hline
CCR                                 & 4948.01                          & 7.49                                    & 0.058                                 \\ \hline
CL                                 & 4941.25                          & 0.73                                    & 0.866                                 \\ \hline
CCY                       & 4945.51                          & 5.00                                    & 0.172                                \\ \hline
RCS                        & 4942.33                          & 1.81                                    & 0.613                                 \\ \hline
MR                              & 4951.91                          & 11.40                                   & \textbf{0.010}                                 \\ \hline
RCE                             & 4991.79                          & 51.28                                   & \textbf{0.000}                                 \\ \hline
PFRC                   & 4950.93                          & 10.41                                    & \textbf{0.015}                                \\ \hline
RI                            & 4951.60                         & 11.086                                    & \textbf{0.011}                                 \\ \hline
INF                                & 4946.96                          & 6.44                                    & 0.092                                \\ \hline
IBF                                 & 4944.99                          & 4.47                                    & 0.215                                \\ \hline
\end{tabular}

==> tables/mlr_combined_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{l|rr|rr|rr|rr}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Variable}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Likelihood\\ ratio test\end{tabular}}      & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Distinguish between\\ False Positive and \\ Functional class\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Distinguish between \\ Evolvability and \\ Functional class\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Distinguish between \\ Discussion and \\ Functional class\end{tabular}} \\ \cline{2-9} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{\textbf{$\chi^2$}} & \multicolumn{1}{l|}{\textit{\textbf{p-value}}} & \multicolumn{1}{c|}{\textbf{$\beta$}}                      & \multicolumn{1}{c|}{\textit{\textbf{p-value}}}                     & \multicolumn{1}{c|}{\textbf{$\beta$}}                     & \multicolumn{1}{c|}{\textit{\textbf{p-value}}}                     & \multicolumn{1}{c|}{\textbf{$\beta$}}                    & \multicolumn{1}{c}{\textit{\textbf{p-value}}}                    \\ \hline
WRC                                            & \multicolumn{1}{r|}{4.706}               & 0.195                                          & \multicolumn{1}{r|}{.555}                            & .647                                                               & \multicolumn{1}{r|}{-1.430}                         & .187                                                               & \multicolumn{1}{r|}{-1.633}                        & .196                                                             \\ \hline
PN                                             & \multicolumn{1}{r|}{3.31}                & 0.346                                          & \multicolumn{1}{r|}{.014}                            & .163                                                               & \multicolumn{1}{r|}{.005}                           & .425                                                               & \multicolumn{1}{r|}{-.002}                         & .777                                                             \\ \hline
CV                                             & \multicolumn{1}{r|}{110.36}              & \textbf{0.000}                                 & \multicolumn{1}{r|}{1.374}                           & \textbf{.000}                                                      & \multicolumn{1}{r|}{1.847}                          & \textbf{.000}                                                      & \multicolumn{1}{r|}{.706}                          & \textbf{.004}                                                    \\ \hline
CCR                                            & \multicolumn{1}{r|}{7.49}                & 0.058                                          & \multicolumn{1}{r|}{.000}                            & .782                                                               & \multicolumn{1}{r|}{.000}                           & .051                                                               & \multicolumn{1}{r|}{.000}                          & .873                                                             \\ \hline
CL                                             & \multicolumn{1}{r|}{0.73}                & 0.866                                          & \multicolumn{1}{r|}{.000}                            & .922                                                               & \multicolumn{1}{r|}{.000}                           & .814                                                               & \multicolumn{1}{r|}{.000}                          & .416                                                             \\ \hline
CCY                                            & \multicolumn{1}{r|}{5.00}                & 0.172                                          & \multicolumn{1}{r|}{-.001}                           & .082                                                               & \multicolumn{1}{r|}{-.001}                          & .059                                                               & \multicolumn{1}{r|}{-.001}                         & .129                                                             \\ \hline
RCS                                            & \multicolumn{1}{r|}{1.81}                & 0.613                                          & \multicolumn{1}{r|}{-.014}                           & .418                                                               & \multicolumn{1}{r|}{-.040}                          & .531                                                               & \multicolumn{1}{r|}{-.044}                         & .734                                                             \\ \hline
MR                                             & \multicolumn{1}{r|}{11.40}               & \textbf{0.010}                                 & \multicolumn{1}{r|}{-.001}                           & .197                                                               & \multicolumn{1}{r|}{-.001}                          & \textbf{.007}                                                      & \multicolumn{1}{r|}{.000}                          & .953                                                             \\ \hline
RCE                                            & \multicolumn{1}{r|}{51.28}               & \textbf{0.000}                                 & \multicolumn{1}{r|}{.000}                            & \textbf{.000}                                                      & \multicolumn{1}{r|}{.000}                           & .368                                                               & \multicolumn{1}{r|}{.000}                          & \textbf{.000}                                                    \\ \hline
PFRC                                           & \multicolumn{1}{r|}{10.41}               & \textbf{0.015}                                 & \multicolumn{1}{r|}{.003}                            & \textbf{.006}                                                      & \multicolumn{1}{r|}{.002}                           & \textbf{.008}                                                      & \multicolumn{1}{r|}{.001}                          & .145                                                             \\ \hline
RI                                             & \multicolumn{1}{r|}{11.086}              & \textbf{0.011}                                 & \multicolumn{1}{r|}{.000}                            & \textbf{.031}                                                      & \multicolumn{1}{r|}{.000}                           & .380                                                               & \multicolumn{1}{r|}{.000}                          & .251                                                             \\ \hline
IBF                                            & \multicolumn{1}{r|}{6.44}                & 0.092                                          & \multicolumn{1}{r|}{-.893}                           & \textbf{.037}                                                      & \multicolumn{1}{r|}{.898}                           & \textbf{.002}                                                      & \multicolumn{1}{r|}{.517}                          & .126                                                             \\ \hline
INF                                            & \multicolumn{1}{r|}{4.47}                & 0.215                                          & \multicolumn{1}{r|}{.138}                            & .700                                                               & \multicolumn{1}{r|}{-.308}                          & .208                                                               & \multicolumn{1}{r|}{-.046}                         & .870                                                             \\ \hline
\end{tabular}
}

==> tables/model_information.tex <==
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{AIC}      & \multicolumn{1}{l|}{\textbf{-2 Log Likelihood}} & \multicolumn{1}{l|}{\textbf{Chi-Square}} & \multicolumn{1}{l|}{\textbf{D.F.}} & \multicolumn{1}{l|}{\textbf{Nagelkerke Pseudo R-Square}} \\ \hline
Null  & 6150.55 & 6150.55                               & ---                             & ---                       & ---                                             \\ \hline
Full  & 4946.51 &  4862.515                               & 1288.04                        & 42                        & 0.429                                           \\ \hline
\end{tabular}


==> tables/primary_project.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Question}                                                                                        & \multicolumn{4}{c|}{\textbf{Open Source Projects}}                       \\ \hline
\multirow{4}{*}{Do you have an open source project that you consider as your primary project ?} & OpenStack (69)   & Ansible (6)   & Kubernetes (3) & Airship (3) \\ \cline{2-5} 
                                                                                                & Linux Kernel (3) & StarlingX (2) & OPNFV (2)      & QEMU (1)    \\ \cline{2-5} 
                                                                                                & Cloud-init (1)   & Istio (1)     & Firefox (1)    & Trident (1) \\ \cline{2-5} 
                                                                                                & Cinder (1)       & Valence (1)   & MariaDB (1)    & Other (20)  \\ \hline
\end{tabular}
